Kernel Mean Matching for Content Addressability of GANs

We propose a novel procedure which adds "content-addressability" to any given unconditional implicit model e.g., a generative adversarial network (GAN). The procedure allows users to control the generative process by specifying a set (arbitrary size) of desired examples based on which similar samples are generated from the model. The proposed approach, based on kernel mean matching, is applicable to any generative models which transform latent vectors to samples, and does not require retraining of the model. Experiments on various high-dimensional image generation problems (CelebA-HQ, LSUN bedroom, bridge, tower) show that our approach is able to generate images which are consistent with the input set, while retaining the image quality of the original model. To our knowledge, this is the first work that attempts to construct, at test time, a content-addressable generative model from a trained marginal model.

==> related_works_note.tex <==

\subsection{Sets as input}
\begin{itemize}
\item Points to make: RNN still relies on ordering. Using symmetric pooling
function requires an end to end training for the feature to be meaningful. 
\item It is not clear how to train or modify an ordinary recurrent neural
network (RNN) to model exchangeable data'' \citep[p. 2]{KorDegHusGalGre2018}. 
\item Alternatively, a simple symmetric function can be used on a set of
features to summarize them into a single vector. PointNet and their
variations \citet{qi2017pointnet} \citet{qi2017pointnet++} use \textbf{max}
pooling to aggregate features from a set of point coordinate. Another
in the image domain - {[}Burst Image Deblurring Using Permutation
Invariant Convolutional Neural Networks, eccv2018{]} takes arbitrary
length images as input in an unordered manner, again with max pooling.%\patsorn{there's
%another paper that use max pooling on features that I can't remember.
%Will add later} A final style representation is \textbf{average}
%from each feature in a set of images in \citet{collomosse2017sketching}.
%So there are at least 3 solutions to process a set of images:
\item Towards a Neural Statistician \citep{EdwSto2016} learns a summary
representative for each dataset from unordered set of data points. 
\item Comparator Networks \citep{XieSheZis2018} 
\item Mention that the form of the mean embeddings matches what is suggested
in Deep Sets \citep{ZahKotRavPocSal2017}. 
\end{itemize}

\subsection{Optimize images based on GAN latent space}
\begin{itemize}
\item Neural image editing \citet{brock2016neural} 
\item Image manifold \citet{zhu2016generative} 
\item \citet{YehCheYiaSchHas2017}. Search GAN's latent for image inpainting 
\end{itemize}

\subsection{Conditional generation}
\begin{itemize}
\item \textcolor{red}{{[}{*}{*}{]}} Conditional Generative Moment-Matching
Networks \citep{RenZhuLiLuo2016}. We will certainly need to comment
on the differences to our approach. Can condition on one image. Their
motivation is not really clear. Loss = norm of the difference between
two conditional embedding operators. Unclear why or what they are
trying to achieve. No KBR. 
\item Conditional Generative Adversarial Nets \citep{MirOsi2014}. Not much
empirical result. 
\item Plug \& Play Generative Networks: Conditional Iterative Generation
of Images in Latent Space \citep{NguCluBenDosYos2017}. Class-conditional
and text-conditional. Gradient ascent in the latent space of a generator
network to maximize the activations of one or multiple neurons in
a separate classifier network. 
\item Compositional GAN: Learning Conditional Image Composition \citep{AzaPatEbrDar2018} 
\end{itemize}

\subsection{Others}
\begin{itemize}
\item Joint Generative Moment-Matching Network for Learning Structural Latent
Code \citep{GaoHua2018}. Also use kernel mean embedding. 
\item Learning Implicit Generative Models with the Method of Learned Moments
\citep{RavMohRosVin2018} 
\item Conditional Density Estimation with Bayesian Normalising Flows \citep{TriTur2018} 
\item Predictive State Recurrent Neural Networks \citep{DowHefLiBooGor2017} 
\item ELEGANT: Exchanging Latent Encodings with GAN for Transferring Multiple
Face Attributes \citep{XiaHonMa2018} 
\end{itemize}

\paragraph{Misc}
\begin{itemize}
\item Training GANs requires a lot of effort. Undocumented tricks. Determining
convergence is non-trivial \citep{MesNowGei2018}. Mode collapse \citep{LinKheFanOh2018,SriValRusGutSut2017,SalGooZarCheRad2016}. 
\item Main goal: turn an ordinary GAN into a conditional version, without
retraining. Give the bedroom use case as an application of the new
approach. We also do not want to have an explicit conditional distribution
model. 
\item Comments on flow-based generative models 
\item Mention that we do not want to rely on sequence modeling techniques
(RNNs) because the set of conditioned images has no order. ``For
example, it is not clear how to train or modify an ordinary recurrent
neural network (RNN) to model exchangeable data'' \citep[p. 2]{KorDegHusGalGre2018}. 
\item IMQ kernel \citep{TolBouGelSch2018}. Inverse multiquadratics kernel. 
\item Use of MMD in the context of GANs. \citet{SutTunStrDeRam2016,LiChaCheYanPoc2017,BinSutArbGre2018} 
\item \wjsay{Consider VAE for the MNIST case. Changing the extractor allows
us to control the generative process, at test time. VAE cannot do
this.} 
\end{itemize}

